Can Neural Networks Understand Logical Entailment?

We introduce a new dataset of logical entailments for the purpose of measuring models' ability to capture and exploit the structure of logical expressions against an entailment prediction task. We use this task to compare a series of architectures which are ubiquitous in the sequence-processing literature, in addition to a new model class---PossibleWorldNets---which computes entailment as a "convolution over possible worlds". Results show that convolutional networks present the wrong inductive bias for this class of problems relative to LSTM RNNs, tree-structured neural networks outperform LSTM RNNs due to their enhanced ability to exploit the syntax of logic, and PossibleWorldNets outperform all benchmarks.

==> ICLR Logic Paper/datasets.tex <==

\section{The Dataset}
\label{appendix-dataset}

\subsection{Dataset requirements}

Our dataset $\mathcal{D}$ is composed of triples of the form
$(A, B, A \entails{} B)$,
where $A \entails{} B$ is 1 if $A$ entails\footnote{Throughout, we focus on \emph{classical} propositional logic, and do not consider e.g., intuitionistic entailment.} $B$, and 0 otherwise.
For example:
\begin{eqnarray*}
(p \wedge q, q, 1) \\
(q \vee r, r, 0)
\end{eqnarray*}

We wanted to ensure that simple baseline models are unable to exploit simple statistical regularities to perform well in this task.
We define a series of baseline models which, due to their structure or the information they have access to, should not be able to solve the entailment recognition problem described in this paper. We distinguish baselines for which we believe there is little chance of them detecting entailment, from those for which there categorically cannot be true modelling of entailment.
The baselines which categorically cannot detect entailment are encoding models which only observe one side of the sequent:
\[
P(A \entails{} B) = \sigma \left(\text{MLP}(f(A))\right) \quad \textrm{or} \quad P(A \entails{} B) = \sigma \left(\text{MLP}(f(B))\right)
\]
where $f$ is a linear bag of words encoder, an MLP bag of words encoder, or a TreeNet.

Because the dataset contains a roughly balanced number of positive and negative examples, it follows that we should expect any model which only sees part of the sequent to perform in line with a random classifier. If they outperform a random baseline on test, there is a structural or symbolic regularity on one side (or both) which is sufficient to identify some subset of positive or negative examples. 
We use these baselines to verify the soundness of the generation process.

Let $\mathcal{D}^+$ and $\mathcal{D}^-$ be the positive and negative entailments:
\begin{eqnarray*}
\mathcal{D}^+ = \{ (A, B) \; | \; (A, B, 1) \in \mathcal{D} \} \\
\mathcal{D}^- = \{ (A, B) \; | \; (A, B, 0) \in \mathcal{D} \}
\end{eqnarray*}


We impose various requirements on the dataset, to rule out  superficial syntactic differences between  $\mathcal{D}^+$ and  $\mathcal{D}^-$ that can be easily exploited by the simple baselines described above.
We require that our classes are balanced:
\begin{eqnarray*}
|\mathcal{D}^+| & = & |\mathcal{D}^-|
\end{eqnarray*}
We do not want there to be any obvious difference in the length of formulas in $\mathcal{D}^+$ and  $\mathcal{D}^-$:
\begin{eqnarray*}
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+} length(A) & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-} length(A) \\
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+} length(B) & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-} length(B) \\
\end{eqnarray*}
We want there to be the same number of new free variables (variables appearing in B that do not appear in A) in both $\mathcal{D}^+$ and  $\mathcal{D}^-$:
\begin{eqnarray*}
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+} |vars(B)-vars(A)| & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-} |vars(B)-vars(A)|
\end{eqnarray*}



Let $num(A, op)$ be the number of occurrences of operator $op$ in formula $A$. So, for example, $num(\neg (p \wedge \neg q), \neg) = 2$. 
We impose the constraint that for each operator $op \in \{\neg, \wedge, \vee, \rightarrow\}$, that
\begin{eqnarray*}
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+}num(A, op) & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-}num(A, op) \\
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+}num(B, op) & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-}num(B, op)
\end{eqnarray*}
Furthermore, we require that the number of occurrences of an operator \emph{at each level in the abstract syntax tree} is the same in $\mathcal{D}^+$ and $\mathcal{D}^-$.
It would not be acceptable if, for example, a typical $B^+$ from $\mathcal{D}^+$ had more disjunctions at the top of the syntax tree than $B^-$ from $\mathcal{D}^-$.
Let $num\_at(B, level, op)$ be the number of occurrences of operator $op$ at $level$ in the syntax tree for $B$. 
We also require that, for each $op$ and $level$:
\begin{eqnarray*}
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+}num\_at(A, level, op) & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-}num\_at(A, level, op) \\
\mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^+}num\_at(B, level, op) & = & \mathop{\mathbb{E}}_{(A,B) \sim \mathcal{D}^-}num\_at(B, level, op)
\end{eqnarray*}

\subsection{Dataset generation}

\subsubsection{A naive approach to dataset generation}

A simple way to generate an entailment dataset would be to alternate between first sampling formulas $A^+$ and $B^+$ such that $A^+ \entails{} B^+$, and second sampling formulas $A^-$ and $B^-$ such that $A^- \notentails{} B^-$.
Since we are alternating between $\entails{}$ and $\notentails{}$, we are guaranteed to produce balanced classes.
Unfortunately, this straightforward approach generates datasets that violate most of our requirements above. 
See Table \ref{dataset-naive} for the details.

In particular, the mean number of negations, conjunctions, and disjunctions at the top of the syntax tree ($num\_at(\cdot, 0, op)$) is markedly different.
$A^+$ has significantly more conjunctions at the top of the syntax tree than $A^-$, while $B^+$ has significantly fewer than $B^-$.
Conversely, $A^+$ has significantly fewer disjunctions at the top of the syntax tree than $A^-$, while $B^+$ has significantly more than $B^-$.

The mean number of satisfying truth-value assignments ($sat(\cdot)$) is also markedly different: $A^+$ is true in on average $3.7$ truth-value assignments (i.e. it is a very specific formula which is only true under very particular circumstances), while $A^-$ is true in $10.3$ truth-value assignments (i.e. it is true in a wider range of circumstances).

If we look at the mean number of variables appearing in $B$ that do not appear in $A$, there is also a striking difference between $\mathcal{D}^+$ and $\mathcal{D}^-$.
The mean number of new variables in $vars(B^+) - vars(A^+)$ is $0.80$ while the mean number of new variables in $vars(B^-) - vars(A^-)$ is $1.39$ with a $\chi^2$ of $3308.1$ and $8$ degrees of freedom. 

We can use these statistics to develop simple heuristic baselines that will be unreasonably effective on the dataset described above:
we can estimate whether $A \entails{} B$ by comparing the lengths of $A$ and $B$, or by looking at the number of variables in $B$ that do not appear in $A$, or by looking at the topmost connective in $A$ and $B$.

\begin{table}[ht]
\centering
\caption{Requirement violations in the naive approach, with $|\mathcal{D}| = 50,000$}
\label{dataset-naive}
\begin{tabular}{lllllllll}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
& {\bf $A^+$} & {\bf $A^-$} & {\bf $\chi^2$} & $\chi^2$ df & {\bf $B^+$} & {\bf $B^-$} & {\bf $\chi^2$} & $\chi^2$ df \\ \hline
{$length(.)$} & 6.62 & 6.45 & 70.6 & 9 & 8.33 & 8.28 & 304.9 & 16 \\
{\bf $num(\cdot, \neg)$} & 1.47 & 1.33 & 309.4 & 8 & 1.77 & 1.91 & 139.0 & 9 \\
{\bf $num(\cdot, \wedge)$} & 1.52 & 1.33 & 308.6 & 8 & 1.70 & 1.94 & 134.0 & 11 \\
{\bf $num(\cdot, \vee)$} & 1.30 & 1.40 & 86.9 & 8 & 1.95 & 1.69 & 127.0 & 10 \\
{\bf $num\_at(\cdot, 0, \neg)$} & 0.31 & 0.22 & 532.4 & 1 & 0.18 & 0.30 &350.9 & 1 \\
{\bf $num\_at(\cdot, 1, \neg)$} & 0.32 & 0.31 & 7.5 & 2 & 0.39 & 0.41 & 3.2 & 2 \\
{\bf $num\_at(\cdot, 2, \neg)$} & 0.31 & 0.31 & 8.8 & 4 & 0.56 & 0.54 & 5.3 & 4 \\
{\bf $num\_at(\cdot, 0, \wedge)$} & {\color{red} 0.35} & {\color{red} 0.2} & 1382.9 & 1 & {\color{red} 0.13} & {\color{red} 0.33} & 1076.4 & 1 \\
{\bf $num\_at(\cdot, 1, \wedge)$} & 0.32 & 0.31 & 36.5 & 2 & 0.39 & 0.40 & 6.5 & 2 \\
{\bf $num\_at(\cdot, 2, \wedge)$} & 0.31 & 0.32 & 3.2 & 4 & 0.56 & 0.53 & 16.5 & 4 \\
{\bf $num\_at(\cdot, 0, \vee)$} & {\color{red} 0.16} & {\color{red} 0.28} & 1070.3 & 1 & {\color{red} 0.34} & {\color{red} 0.16} & 752.4 & 1 \\
{\bf $num\_at(\cdot, 1, \vee)$} & 0.30 & 0.32 & 66.0 & 2 & 0.42 & 0.34 & 141.1 & 2 \\
{\bf $num\_at(\cdot, 2, \vee)$} & 0.32 & 0.31 & 12.9 & 4 & 0.57 & 0.52 & 39.7 & 4 \\
{\bf $\#sat(\cdot)$} & {\color{red} 3.7} & {\color{red} 10.3} & 11265 & 174 & {\color{red} 22.1} & {\color{red} 11.7} & 3702.8 & 241 \\ \hline
\end{tabular}
\end{table}

\subsubsection{Our preferred approach to dataset generation}

In order to satisfy our requirements above, we took a different approach to dataset generation.
In order to ensure that there are no crude statistical measurements that can detect differences between $\mathcal{D}^+$ and $\mathcal{D}^-$, we change the generation procedure so that every formula appears in both $\mathcal{D}^+$ and $\mathcal{D}^-$.
We sample 4-tuples of formulas $(A_1, B_1, A_2, B_2)$ such that:
\begin{eqnarray*}
A_1 & \entails{} & B_1 \\
A_2 & \entails{} & B_2 \\
A_1 & \notentails{} & B_2 \\
A_2 & \notentails{} & B_1
\end{eqnarray*}
Here, each of the four formulas appears in one positive entailment and one negative entailment\footnote{One consequence of this method is that it rules out $A_1$ from being impossible (if it was impossible, we would not have $A_1 \notentails{} B_2$) and $B_1$ from being a tautology (if it was a tautology, we would not have $A_2 \notentails{} B_1)$.}.

Using this alternative approach, we are able to satisfy the requirements above.
By construction, the mean length, number of operators at a certain level in the syntax tree, and the number of satisfying truth-value assignments is \emph{exactly the same} for $\mathcal{D}^+$ and $\mathcal{D}^-$.
See Table \ref{dataset-preferred}.

The only crude difference remaining is in the number of new variables.
If we look at the number of variables appearing in $B$ that do not appear in $A$, there is a noticeable difference between $\mathcal{D}^+$ and $\mathcal{D}^-$.
The mean number of new variables in $vars(B^+) - vars(A^+)$ is $1.25$ while the mean number of new variables in $vars(B^-) - vars(A^-)$ is $1.60$ with a $\chi^2$ of $922.1$ and $8$ degrees of freedom. 

\begin{table}[ht]
\centering
\caption{Statistics for the preferred approach that generates 4-tuples, with $|\mathcal{D}| = 50,000$}
\label{dataset-preferred}
\begin{tabular}{lllllllll}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
& {\bf $A^+$} & {\bf $A^-$} & {\bf $\chi^2$} & $\chi^2$ df & {\bf $B^+$} & {\bf $B^-$} & {\bf $\chi^2$} & $\chi^2$ df \\ \hline
{$length(.)$} & 6.33 & 6.33 & 0.0 & 9 & 6.38 & 6.38 & 0.0 & 16 \\
{\bf $num(\cdot, \neg)$} & 1.42 & 1.42 & 0.0 & 9 & 1.26 & 1.26 & 0.0 & 8 \\
{\bf $num(\cdot, \wedge)$} & 1.63 & 1.63 & 0.0 & 7 & 1.16 & 1.16 & 0.0 & 7 \\
{\bf $num(\cdot, \vee)$} & 1.14 & 1.14 & 0.0 & 7 & 1.53 & 1.53 & 0.0 & 8 \\
{\bf $num\_at(\cdot, 0, \neg)$} & 0.33 & 0.33 & 0.0 & 1 & 0.16 & 0.16 & 0.0 & 1 \\
{\bf $num\_at(\cdot, 1, \neg)$} & 0.29 & 0.29 & 0.0 & 2 & 0.32 & 0.32 & 0.0 & 2 \\
{\bf $num\_at(\cdot, 2, \neg)$} & 0.30 & 0.30 & 0.0 & 3 & 0.31 & 0.31 & 0.0 & 4 \\
{\bf $num\_at(\cdot, 0, \wedge)$} & 0.49 & 0.49 & 0.0 & 1 & 0.1 & 0.1 & 0.0 & 1 \\
{\bf $num\_at(\cdot, 1, \wedge)$} & 0.34 & 0.34 & 0.0 & 2 & 0.31 & 0.31 & 0.0 & 2 \\
{\bf $num\_at(\cdot, 2, \wedge)$} & 0.30 & 0.30 & 0.0 & 4 & 0.30 & 0.30 & 0.0 & 4 \\
{\bf $num\_at(\cdot, 0, \vee)$} & 0.08 & 0.08 & 0.0 & 1 & 0.39 & 0.39 & 0.0 & 1 \\
{\bf $num\_at(\cdot, 1, \vee)$} & 0.27 & 0.27 & 0.0 & 2 & 0.35 & 0.35 & 0.0 & 2 \\
{\bf $num\_at(\cdot, 2, \vee)$} & 0.29 & 0.29 & 0.0 & 3 & 0.29 & 0.29 & 0.0 & 3 \\
{\bf $\#sat(\cdot)$} & 3.86 & 3.86 & 0.0 & 86 & 14.42 & 14.42 & 0.0 & 157 \\ \hline
\end{tabular}
\end{table}

\subsection{Dataset Example}

Our method generates 4-tuples such as the following:
\begin{eqnarray*}
p \vee p & \entails{} & (r \rightarrow c) \rightarrow ((r \rightarrow v) \vee p) \\
((g \vee p) \vee s) \rightarrow (g \rightarrow g) \wedge r & \entails{} & r \wedge (r \rightarrow r) \\
p \vee p & \notentails{} & r \wedge (r \rightarrow r) \\
((g \vee p) \vee s) \rightarrow (g \rightarrow g) \wedge r & \notentails{} & (r \rightarrow c) \rightarrow ((r \rightarrow v) \vee p)
\end{eqnarray*}

